Topological States of Matter in Frustrated Quantum Magnetism

Frustrated quantum magnets may exhibit fascinating collective phenomena. The main goal of this dissertation is to provide conclusive evidence for the emergence of novel phases of matter like quantum spin liquids in local quantum spin models. We develop novel algorithms for large-scale Exact Diagonalization computations. Sublattice coding methods for efficient use of lattice symmetries in the procedure of diagonalizing the Hamiltonian matrix are proposed and suggest a randomized distributed memory parallelization strategy. Benchmarks of computations on various supercomputers with system size up to 50 spin-1/2 particles have been performed. Results concerning the emergence of a chiral spin liquid in a frustrated kagome Heisenberg antiferromagnet are presented. The stability and extent of this phase are discussed. In an extended Heisenberg model on the triangular lattice, we establish another chiral spin liquid phase. We discuss the special case of the Heisenberg $J_1$-$J_2$ model and present a scenario where the critical point of phase transition from the 120-degree N\'eel to a putative $\mathbf{Z}_2$ spin liquid is described by a Dirac spin liquid. A generalization of the SU(2) Heisenberg model with SU(N) degrees of freedom on the triangular lattice with an additional ring-exchange term is discussed. We present our contribution to the project and the final results that suggest a series of chiral spin liquid phases in an extended parameter range. Finally, we present preliminary data from a Quantum Monte Carlo study of an SU(N) version of the J-Q model on a square lattice for N=2,...,10, and multi-column representations. We establish the phase boundary between the N\'eel ordered phase and the disordered phases. The disordered phase in the four-column representation is expected to be a two-dimensional analog of the Haldane phase for the spin-1 Heisenberg chain.

==> chapters/abstract/abstract_english_online_form.tex <==
%auto-ignore
\chapter*{\centering Abstract / Zusammenfassung}
\label{sec:abstract}
Frustrated quantum magnets may exhibit fascinating collective phenomena. The main goal of this dissertation is to provide conclusive evidence for the emergence of novel phases of matter like quantum spin liquids in local quantum spin models. After a general introduction to frustrated magnetism, spin liquids and the numerical methods employed in part I comprising chapter 1 and 2 we present the main results of the thesis in part II.

We develop novel algorithms for large-scale Exact Diagonalization computations in chapter 3. So-called sublattice coding methods for efficient use of lattice symmetries in the procedure of diagonalizing the Hamiltonian matrix are proposed. Furthermore, we suggest a randomized distributed memory parallelization strategy. Benchmarks of computations on various supercomputers with system size up to 50 spin-1/2 particles have been performed.

Results concerning the emergence of a chiral spin liquid in a frustrated kagome Heisenberg antiferromagnet are presented in chapter 4. We confirm previous findings obtained via DMRG calculations using Exact Diagonalization and propose that the chiral spin liquid phase in this model is well described by Gutzwiller-projected wave functions. Also, the stability and extent of this phase are discussed. 

In an extended Heisenberg model on the triangular lattice, we establish another chiral spin liquid phase in chapter 5 amongst several magnetically ordered phases. We discuss the special case of the Heisenberg J_1-J_2 model with nearest and next-nearest neighbor interactions and present a scenario where the critical point of phase transition from the 120 degree Néel to a putative Z_2 spin liquid is described by a Dirac spin liquid.

A generalization of the SU(2) Heisenberg model with SU(N) degrees of freedom on the triangular lattice with an additional ring-exchange term is discussed in chapter 6. We present our contribution to the project and the final results that suggest a series of chiral spin liquid phases in an extended parameter range for N=3,...,10. 

Finally, we present preliminary data from a Quantum Monte Carlo study of an SU(N) version of the J-Q model on a square lattice in chapter 7. We study this model for N=2,...,10 and multi-column representations of SU(N) and establish the phase boundary between the Néel ordered phase and the disordered phases for J, Q >= 0. The disordered phase in the four-column representation is expected to be a two-dimensional analog of the Haldane phase for the spin-1 Heisenberg chain.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../thesis"
%%% End:


==> chapters/abstract/abstract_german_online_form.tex <==
%auto-ignore
% \chapter*{\centering Zusammenfassung}
% \label{sec:abstract_german}

\subsubsection{Deutsche Zusammenfassung}
Frustrierte Quantenmagnete können faszinierende kollektive Phänomene aufweisen. Das Ziel dieser Dissertation ist es schlüssigen Nachweis für die Emergenz neuer Materiezustände wie Quantenspinflüssigkeiten in lokalen Quantenspinmodellen zu erbringen. Nach einer allgemeinen Einleitung in frustrierten Magnetismus, Spinflüssigkeiten und die verwendeten numerischen Methoden in Teil I, bestehend aus Kapitel 1 und 2 stellen wir die wichtigsten Ergebnisse dieser Arbeit in Teil II vor.

Wir entwickeln neue Algorithmen für skalierbare Exakte Diagonalisierung in Kapitel 3. So genannte Untergitterkodierungsmethoden zur effizienten Nutzung von Gittersymmetrien im Vorgang der Diagonalisierung der Hamiltonmatrix werden vorgeschlagen. Desweiteren stellen wir eine randomisierte Parellelisierungsstrategie für verteilte Speichersysteme vor. Benchmarks mit Systemgrößen bis zu 50 Spin-1/2 Teilchen wurden auf mehreren Supercomputern durchgeführt.

Ergebnisse zur Emergenz von chiralen Spinflüssigkeiten in einem erweiterten Heisenberg Antiferromagneten auf dem Kagome-Gitter werden in Kapitel 4 vorgestellt. Wir bestätigen vorangegangene DMRG Studien mithilfe der Exakten Diagonalisierung und zeigen auf, dass diese chirale Spinflüssigkeit gut mithilfe Gutzwiller-projizierter Wellenfunktionen beschrieben werden kann.  Desweiteren werden die Stabilität und die Ausdehnung dieser Phase behandelt.

In einem erweiterten Heisenbergmodell auf dem Dreiecksgitter bringen wir den Nachweis einer weiteren chiralen Spinflüssigkeitsphase zwischen mehreren magnetisch geordneten Phasen in Kapitel 5. Wir besprechen den Spezialfall des Heisenberg J_1-J_2 Modells mit nächster- und übernächster-Nachbar Wechselwirkung und stellen ein Szenario vor, bei welchem der kritische Punkt des Phasenübergangs zwischen der 120 Grad Néel geordneten und der mutmaßlichen Z_2 Spinflüssigkeit durch eine Dirac Spinflüssigkeit beschrieben wird.

Eine Verallgemeinerung des SU(2) Heisenberg Modells mit SU(N) Freiheitsgraden auf dem Dreiecksgitter mit zusätzlichem Ringaustauschterm wird in Kapitel 6 diskutiert. Wir stellen unseren Beitrag zum Projekt und die endgültigen Ergebnisse vor, welche eine Reihe von chiralen Spinflüssigkeitsphasen in einer ausgedehnten Parameterregion für N=3,...,10.

Zuletzt stellen wir vorläufige Daten einer Quanten Monte Carlo Studie zu einer SU(N) Version des J-Q Modells auf dem Quadratgitter vor.  Wir untersuchen dieses Modell für N=2,...,6 und Darstellungen mit mehreren Spalten von SU(N) und stellen den Phasenübergangspunkt von der Néel geordneten zur ungeordeten Phase für J, Q >= 0 fest. Es wird erwartet, dass die ungeordnete Phase in der vier-Spalten Darstellung ein zweidimensionales Analogon zur Haldane Phase der Spin-1 Heisenberg Kette ist.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../thesis"
%%% End:


==> chapters/exact_diagonalization/exact_diagonalization.tex <==
%auto-ignore

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 
\subsection{Exact Diagonalization}
\subsubsection{Lanczos Algorithms}
asdf
\subsubsection{Using Symmetries of the Hamiltonian}
A symmetry of the System is an operator $\mathcal{S}$ that commutes with the
Hamiltonian $\mathcal{H}$, i.e. $[\mathcal{H},\mathcal{S}]=0$. Given a symmetry
of the Hamiltonian we can choose a basis $\left( \ket{\psi^S_i}\right)$ of the
Hilbertspace, such that all states in this new basis are eigenstates
of the operator $\mathcal{S}$. Of course for arbitrary symmetries finding this
basis amounts to fully diagonalizing the $\mathcal{S}$ operator. 

Consider for example the Spin-$1/2$ Heisenberg model on an arbitrary
lattice
\[
\mathcal{H} = \sum\vec{S}_i\cdot\vec{S}_j
\]
This model has a $\mathbb{Z}_2$ spinflip symmetry. The operator
\[
\mathcal{S}_{\textnormal{flip}} = \sigma^x_1 \sigma^x_2 \cdots \sigma^x_N 
\]
flipping all spins on the lattice simulateously commutes with the
Heisenberg Hamiltonian. For this symmetry we can readily write down 
a basis in which this operator is diagonal. For each spin
configuration $\ket{\vec{\sigma}} \equiv \ket{\sigma_1, \sigma_2, \cdots, \sigma_N}$
the two states
\begin{align*}
  \ket{\vec{\sigma}} _{\textnormal{even}} = \ket{\vec{\sigma}} + 
  \mathcal{S}_{\textnormal{flip}}\ket{\vec{\sigma}} \\
  \ket{\vec{\sigma}} _{\textnormal{odd}} = \ket{\vec{\sigma}} - 
  \mathcal{S}_{\textnormal{flip}}\ket{\vec{\sigma}} 
\end{align*}
are eigenstates of the operator $\mathcal{S}_{\textnormal{flip}}$ with
eigenvalues $\pm 1$. Moreover the Heisenberg Hamiltonian $\mathcal{H}$
will be blockdiagonal in this new basis. The parity with respect to
the spinflip symmetry is a conserved quantity.

Similarly given our model has a translational symmetry (e.g.by
assuming periodic boundary conditions on a torus) by a vector $\vec{t}$
\[
\mathcal{T} \ket{\sigma_{\vec{p}_1}, \sigma_{\vec{p}_2}, \cdots, \sigma_{\vec{p}_N}} = 
  \ket{\sigma_{{\vec{p}_1} - \vec{t}}, \sigma_{{\vec{p}_2} - \vec{t}}, \cdots, \sigma_{{\vec{p}_N} - \vec{t}}}
\]
we can also write down a new basis in which $\mathcal{T}$ is
diagonal. For a spin configuration $\ket{\vec{\sigma}}$ the states
\begin{equation}
  \label{eq:blochstateonlytranslation}
  \ket{\vec{\sigma}}_{\vec{k}} = \sum\limits_{\mathcal{T} }
  e^{i\vec{k}\cdot\vec{t}}\mathcal{T} \ket{\vec{\sigma}}
\end{equation}
where the sum runs over all translations of the lattice including the
identity defines this new basis.  
 
\subsubsection{Sublattice Coding Techniques}
In the previous section we have seen that in order to efficiently use
lattice and certain onsite symmetries in exact diagonalization
calculations we have to work in a symmetrized basis of the
Hilbertspace which block-diagonalizes the Hamiltonian. Then 
Lanczos algorithms can be applied to perform eigenvalue computations
on the individual blocks. In this section we describe how to
represent this basis in a computer and how the Hamiltonian is
expressed in this representation. Moreover we identify the key
algorithmic challenge of working in these bases and propose methods
to face those in a fast and memory efficient manner, the so called
\textit{sublattice coding techniques}.

We consider a lattice Spin-Hamiltonian of the form
\[
\mathcal{H} = \sum\limits_i H_i
\]
where the $H_i$ are non-branching bonds, i.e. 
\begin{equation}
  \label{eq:nonbranchingcondition}
  H_i\ket{\vec{\sigma}} = c_{i}(\vec{\sigma})\ket{\vec{\tau}}
\end{equation}
the point being that the right hand side of
eq. \eqref{eq:nonbranchingcondition} is a single spin configuration
and no linear combination of different spin configurations.
Note that this is no restriction on the class of Hamiltonians we consider but
only a way of expressing them. For example a simple Spin $1/2$
Heisenberg bond $\vec{S}_i\cdot \vec{S}_j$ does not fulfill the above 
condition but it can be rewritten as a sum of a spin exchange 
bond $\frac{1}{2}\left( S_i^+S_j^- + S_i^-S_j^+\right)$ and an Ising
bond $S_i^z S_j^z$ which do indeed fulfill the non-branching
condition individually.

\todo{explain problem of finding a representative}
For a given one-dimensional representation $\mathcal{R}$ of the symmetry group the
symmetrized states are given by 
\begin{equation}
  \label{eq:defsymmetrizedstate}
  \ket{\vec{\sigma}_{\textnormal{sym}}} = \frac{1}{\mathcal{N}}\sum\limits_{
    s \in \mathcal{S}_\Lambda} \chi^{\mathcal{R}}(s) s\left(\ket{\vec{\sigma}}\right)
\end{equation}
where $\chi^{\mathcal{R}} (s)$ is the character of the representation
$\mathcal{R}$. In order to work in the basis of the symmetrized states
we need to know the matrix elements of the Hamiltonian in this basis. 

\[
\braket{\vec{\tau}_{\textnormal{sym}}| \mathcal{H} |
\vec{\sigma}_{\textnormal{sym}}}
\]

The action of all symmetry group elements on a given spinstate
$\ket{\vec{\sigma}}$ creates several different states which we will
call the orbit $\mathcal{O}\left(\ket{\vec{\sigma}}\right)$ of
$\ket{\vec{\sigma}}$. In order to represent the
symmetrized state in equation \eqref{eq:defsymmetrizedstate} on
a computer one element, i.e. one particular spin configuration of this
orbit is chosen and called the \textit{representative}
$\ket{\vec{\sigma}}_{\textnormal{R}}$. Although this
choice is arbitrary we will always choose the smallest element of the
orbit with respect to  the integer coding as the representative:
\begin{equation}
  \label{eq:deforbitrepresentative}
  \ket{\vec{\sigma}}_{\textnormal{R}} = \argmin\limits_{\ket{\vec{\tau}} \in
  \mathcal{O}\left(\ket{\vec{\sigma}}\right)} \textnormal{int}\left(\ket{\vec{\tau}}\right)
\end{equation}
It turns out that the task of finding the representative for a given
spin configuration is the central computational challenge. 

In order to explain our algorithm we first have to introduce some nomenclature.
\begin{defn}[Sublattice stability]
  A lattice $\Lambda$ with spatial symmetry group
  $\mathcal{S}_\Lambda$ is called $k$-\textit{sublattice stable} if there exists
  a decomposition of $\Lambda$ into $k$ disjoint subsets 
  \[
  \Lambda_k \subset \Lambda  \textnormal{ with } 
  \Lambda = \bigcupdot\limits_k \Lambda_k
  \]
  such that every $s\in \mathcal{S}_\Lambda$ maps each $\Lambda_k$
  onto exactly one (possibly different) $\Lambda_l$, i.e. for all 
  $s\in \mathcal{S}_\Lambda$ and all $\Lambda_k$ there exists a 
  $\Lambda_l$ such that 
  \[
  s(\Lambda_k) = \Lambda_l.
  \]
  The set $\Lambda_k$ is called the $k$-\textit{sublattice} of $\Lambda$.
\end{defn}


\begin{figure}[t!]
    \centering
    \begin{minipage}[c]{0.3\textwidth}
        \includegraphics[width=\textwidth]{linearchain}
    \end{minipage}%
    \quad
    \begin{minipage}[c]{0.3\textwidth}
      \includegraphics[width=\textwidth]{kagome}
    \end{minipage}
    \quad
    \begin{minipage}[c]{0.3\textwidth}
      \quad
      \includegraphics[width=0.9\textwidth]{square}
    \end{minipage}
    \\
    \begin{minipage}[t]{0.3\linewidth}
      \subcaption{Two sublattice ordering in a linear chain.
            \label{fig:sublatticeorderings:linearchain}}
    \end{minipage}
    \quad
    \begin{minipage}[t]{0.3\linewidth}
      \subcaption{Three sublattice ordering on a kagomé lattice.
        \label{fig:sublatticeorderings:kagome}}
    \end{minipage}
    \quad
    \begin{minipage}[t]{0.3\linewidth}
      \subcaption{Three sublattice ordering on a square lattice.       
        \label{fig:sublatticeorderings:square}}
    \end{minipage}

\caption{Sublattice orderings for several common lattices. In figures
  \ref{fig:sublatticeorderings:linearchain} and 
  \ref{fig:sublatticeorderings:kagome} the sublattices
  are stable with respect to all spatial symmetries. In figure
  \ref{fig:sublatticeorderings:square} the sublattices are stable
  with respect to all translational symmetries,
  horizontal and vertical reflections, $180^\circ$ rotations but not
  with respect to $90^\circ$ rotations or diagonal reflections.}
  \label{fig:sublatticeorderings}
\end{figure}

\begin{exmpl}
  The notion of \textit{sublattice stability} is illustrated in
  Fig.~\ref{fig:sublatticeorderings}. The sublattices $\Lambda_k$ are
  drawn in different colors. A  translation by one lattice site in Fig.
  \ref{fig:sublatticeorderings:linearchain} exchanges the sublattices.
  A $60^\circ$ rotation around a hexagon center in Fig.
  \ref{fig:sublatticeorderings:kagome} for example cyclically permutes
  the three sublattices. One checks that for both
  Figs.~\ref{fig:sublatticeorderings:linearchain},~\ref{fig:sublatticeorderings:kagome} 
  all translational as well as
  all pointgroup symmetries are sublattice stable, so different color
  sublattices are mapped onto each other. This is different for 
  Fig.~\ref{fig:sublatticeorderings:square}. Still here all translational
  symmetries just permute the sublattices, but a $90^\circ$ rotation
  splits up a sublattice into different sublattices. Nevertheless a
  $180^\circ$ rotation keeps the sublattices stable, similarly a
  vertical or horizontal reflection. Therefore only the reduced pointgroup $D2$
  instead of the full $D4$ pointgroup for the square lattice fulfills
  the sublattice stability condition in this case. Note that for a
  square lattice one can easily choose a two or four sublattice
  decomposition for which the full $D4$ pointgroup is sublattice stable.
\end{exmpl}

For a decomposition of a lattice $\Lambda$ into stable sublattices
$\Lambda_1, \cdots, \Lambda_k$ also the symmetries of the lattice can
be decomposed into $k$ classes.

\begin{defn}
  Given a lattice  $\Lambda$ with spatial symmetry group
  $\mathcal{S}_\Lambda$ which is $k$-sublattice stable with
  sublattices $\Lambda_1, \cdots, \Lambda_k$, then every symmetry $s \in
  \mathcal{S}_\Lambda$ maps a sublattice $\Lambda_l$ onto 
  $\Lambda_1$, i.e.
  \begin{equation}
    \label{eq:sublatticesymmetrydefinition}
    s(\Lambda_l) = \Lambda_1. 
  \end{equation}
 A spatial symmetry mapping the sublattice $\Lambda_l$ to  $\Lambda_1$ is
 called an \textbf{$l$-symmetry}. The set of all $l$-symmetries is
 denoted by $\mathcal{S}_\Lambda^l$

\end{defn}
There are thus $k$ classes of symmetries for a $k$-sublattice stable
lattice. Finally we now want to introduce the convention that spin states
$\ket{\vec{\sigma}}$ are labeled as
\begin{equation}
  \label{eq:sublatticespinstatelabel}
  \ket{\vec{\sigma}} = \ket{\underbrace{\sigma_1,\cdots,
      \sigma_{N/k}}_{\Lambda_1},\underbrace{\sigma_{N/k + 1},\cdots,
      \sigma_{2N/k}}_{\Lambda_2}, \cdots, \underbrace{\sigma_{(k-1)N/k},\cdots,
      \sigma_{N}}_{\Lambda_k} }
\end{equation}
i.e. the first $N/k$ spins are on the sublattice $\Lambda_1$, the
second $N/k$ spins on sublattice $\Lambda_2$ and so on. Fig. 
\ref{fig:123symmetriesaction} shows how the different $l$-symmetries
now act on the spinstates. An $l$-symmetry maps a spin configuration
on sublattice $\Lambda_l$ to the sublattice $\Lambda_1$.  


\begin{figure}
  \centering
  \tikzset{
    % Define standard arrow tip
    >=stealth',
    % Define arrow style
    pil/.style={
      ->,
      thick,
      shorten <=2pt,
      shorten >=2pt,}
  }

  \begin{tikzpicture}[node distance=1cm, auto,]
    % nodes

    \node[](a_sublattice){
      $\ket{\textcolor{orange}{\uparrow \downarrow \downarrow\uparrow} 
        \; \textcolor{black}{\downarrow\uparrow \downarrow \uparrow}
        \; \textcolor{black}{\uparrow \uparrow \downarrow
          \downarrow}}$};

    \node[below=0.5cm of a_sublattice](b_sublattice)
    { $\ket{\textcolor{black}{\uparrow \downarrow \downarrow\uparrow} 
        \; \textcolor{orange}{\downarrow\uparrow \downarrow \uparrow}
        \; \textcolor{black}{\uparrow \uparrow \downarrow \downarrow}}$};

    \node[below=0.5cm of b_sublattice](c_sublattice) {
      $\ket{\textcolor{black}{\uparrow \downarrow \downarrow\uparrow}
        \; \textcolor{black}{\downarrow\uparrow \downarrow \uparrow}
        \; \textcolor{orange}{\uparrow \uparrow \downarrow \downarrow}}$};

    \node[right=2.5cm of b_sublattice](result){
      $\ket{\textcolor{orange}{\uparrow \downarrow \uparrow \downarrow} 
        \; \textcolor{black}{\downarrow \downarrow \uparrow \uparrow}
        \; \textcolor{black}{\uparrow  \downarrow \downarrow \uparrow}}$};
     
        \path[->](a_sublattice) edge [bend left] node [above left=0.1 cm
        of result] {$1$-symmetry} (result) ;
        \path[->](b_sublattice) edge node {$2$-symmetry} (result) ;
        \path[->](c_sublattice) edge [bend right] node [below left=0.1cm
        of result]{$3$-symmetry}  (result);

  \end{tikzpicture}
  \caption{Action of $l$-symmetries on ordered spin configurations.}
  \label{fig:123symmetriesaction}
\end{figure}

With this definitions and nomenclature we are now ready to describe
the sublattice coding algorithm for finding the representative 
$\ket{\vec{\sigma}}_{\textnormal{R}} $ as defined in eq. \eqref{eq:deforbitrepresentative}
Of a given spin configuration $\ket{\vec{\sigma}}$. The main task is
to find the minimal spinconfiguration in eq. \eqref{eq:deforbitrepresentative}. 

\RestyleAlgo{boxruled}
\LinesNumbered
\begin{algorithm}[ht]
  \caption{Finding the representative
    $\ket{\vec{\sigma}}_{\textnormal{R}}$ given $\Ket{\vec{\sigma}}$}
  Split up the spin configuration $\ket{\vec{\sigma}}$ into configurations on the
  individual sublattices $\ket{\vec{\sigma}}^l$. \\
  Look up the representatives $\ket{\vec{\sigma}}^l_{\textnormal{R}} $
  of the states $\ket{\vec{\sigma}}^l$
  with respect to the $l$-symmetries $\mathcal{S}_\Lambda^l$ and 
  look up all symmetries that lead to this representative. \\
  The minimal representative $\ket{\vec{\sigma}}^l_{\textnormal{R}}$ 
  will constitute the leading spin configuration in the
  representative $\ket{\vec{\sigma}}_{\textnormal{R}}$. Decide which 
  representatives $\ket{\vec{\sigma}}^l_{\textnormal{R}}$ are
  minimal. In general this can be more than one.\\
  For every $l$ for which $\ket{\vec{\sigma}}^l_{\textnormal{R}}$ is
  minimal apply the symmetries which lead to this representative to
  the whole spinconfiguration $\ket{\vec{\sigma}}$. The true 
  representative $\ket{\vec{\sigma}}_{\textnormal{R}}$ is the minimal
  amongst the states created by applying this symmetries.
\label{alg:findrepresentativesublattices}
\end{algorithm}

  \begin{figure}
    \centering
    \tikzset{
      % Define standard arrow tip
      >=stealth',
      % Define arrow style
      pil/.style={
        ->,
        thick,
        shorten <=2pt,
        shorten >=2pt,}
    }
 
  \begin{tikzpicture}[node distance=1cm, auto,]
      % nodes
      \node[](original_spinconfiguration){
        $\ket{\vec{\sigma}}=\ket{1101 \; 1000}  $};

      \node[above right=1 cm and -0.3cm
      of original_spinconfiguration](AWord){
        $\ket{\vec{\sigma}}^1=\ket{1101}  $};

      \node[below right=1 cm and -0.3cm
      of original_spinconfiguration](BWord){
        $\ket{\vec{\sigma}}^2=\ket{1000}  $};


      \node[right=1.5 cm of AWord](ARep){
        $\ket{\vec{\sigma}}_{\textnormal{R}}^1= \ket{0111}  $};
      \node[right=1.5 cm of BWord](BRep){
        $\ket{\vec{\sigma}}_{\textnormal{R}}^2= \ket{0001}  $};

      \node[below right=1 cm and -0.3cm of ARep](representativeprefix){
        $\ket{\vec{\sigma}}_{\textnormal{R}} =\ket{0001 \; ????}  $};

      \node[below=2.5 cm of representativeprefix](representative){
        $\ket{\vec{\sigma}}_{\textnormal{R}} =\ket{0001 \; 1011}  $};
      
      \path[->](original_spinconfiguration) edge node {\textbf{1}} (AWord) ;
      \path[->](original_spinconfiguration) edge (BWord) ;
      \path[->](AWord) edge node {\textbf{2}} (ARep) ;
      \path[->](BWord) edge (BRep) ;
      \path[->](ARep) edge node  {\textbf{3}} (representativeprefix) ;
      \path[->](BRep) edge (representativeprefix) ;
      \path[->](representativeprefix) edge node {\textbf{4}} (representative) ;
    \end{tikzpicture}

    \caption{Example and basic idea of the sublattice coding algorithm for two
      sublattices. The edge labels 1-4 of the diagram correspond to
      the steps 1-4 in algorithm~\ref{alg:findrepresentativesublattices}.
    }
    \label{fig:sublatticealgorithm}
  \end{figure}




\subsubsection{Parallelization for distributed memory machines}
asdf

\subsubsection{Benchmarks}
\begin{table}[ht!]
  \tiny \centering
  \begin{tabular}{|c | c | c | c | c | c | c |}
    \hline
    Testproblem & \# sites & Sym. sector & Dimension & \# of cores & Time creating H. space &
                                                                                              Time per Lanczos iteration \\
    \hline
    \hline 
    \multicolumn{7}{|l|}{\textbf{Benchmarks on VSC3}} \\
    \hline 

    TFI Square & 40 & $\Gamma$.C4.A &  3436321976 & 512 & 85.1579 secs & 144.88 secs\\
    TFI Square & 40 & X.C2.A &  6871803500 & 512 & 56.6237 secs & 260.11 secs\\
    TFI Square & 40 & 1.C1.A & 13743973884 & 512 & 35.9353 secs & 622.4 secs\\

    HB $J_1J_2$ triangular & 48 & $\Gamma$.D6.A1 & 27994566043 & 8192 & 1011.17 secs & 1026.1 secs \\
    HB $J_1J_2$ triangular & 48 & $\Gamma$.D6.E2 & 55986856310 & 8192 & 412.818 secs & 1859.6 secs \\
    HB NN square & 48 & $\Gamma$.D2.A1 &$ \sim 8.397 \cdot 10 ^{10}$& 8192 &  n.a & 1521.3 secs \\
    HB NN square & 52 & $\Gamma$.C4.A & 1192120347817 & 12288 & 3612.49 secs & n.a. \\
    \hline
    \multicolumn{7}{|l|}{\textbf{Benchmark on RZG Hydra}}\\
    \hline
    HB NN kagome & 48 & $\Gamma$.D6.A1 & 83979009353 &  10240 & 317.507 secs & 257.98 secs \\
    \hline
  \end{tabular}
  \caption{Benchmark results for various problems on VSC3 and RZG
    Hydra.}
  \label{tab:benchmarks}
\end{table}

\begin{table}[ht!]
  \tiny \centering
  \begin{tabular}{|c | c | c | c | c |}
    \hline
    Testproblem & \# sites & Dimension & \# of cores & Time per Lanczos iteration \\
    \hline
    \hline 
    \multicolumn{5}{|l|}{\textbf{Benchmarks on VSC3}} \\
    \hline 

    TFI Square & 40 & $3.4 \cdot 10 ^{9}$ & 512 & 144.88 secs\\
    TFI Square & 40 & $6.9 \cdot 10 ^{9}$ & 512 & 260.11 secs\\
    TFI Square & 40 & $1.4 \cdot 10 ^{10}$ & 512 & 622.4 secs\\
    HB $J_1J_2$ triangular & 48 & $2.8 \cdot 10 ^{10}$ & 8192 & 1026.1 secs \\
    HB $J_1J_2$ triangular & 48 & $5.6 \cdot 10 ^{10}$ & 8192 & 1859.6 secs \\
    HB NN square & 48 &  $8.4 \cdot 10 ^{10}$ & 8192 & 1521.3 secs \\
    HB NN square & 50 &  $3.1 \cdot 10 ^{11}$ & 8192 & 3834 secs \\
    HB NN square & 52 & $1.2 \cdot 10 ^{12}$ & 12288 & n.a.\\
    \hline
    \multicolumn{5}{|l|}{\textbf{Benchmark on RZG Hydra}}\\
    \hline
    HB NN kagome & 48 & $8.4 \cdot 10 ^{10}$ &  10240 & 257.98 secs \\
    \hline
  \end{tabular}
  \caption{Benchmark results for various problems on VSC3 and RZG
    Hydra.}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../thesis"
%%% End:


==> chapters/hubbard_perturbation/hubbard_perturbation.tex <==
%auto-ignore

\chapter{Effective Spin model from SU($N$) Hubbard model in magnetic field.}
Starting from the SU($N$) Hubbard model in a magnetic field 
\begin{equation}
  \label{eq:sunhubbard}
  H = - \sum \limits_{\left< i, j\right>, \alpha=1} (t_{ij} c_{i,\alpha}^\dagger c_{j,\alpha} +  
  t_{ij}^* c_{j,\alpha}^\dagger  c_{i,\alpha}) + U \sum\limits_{i, \alpha < \beta} n_{i,\alpha} n_{i,\beta} 
      = H_t + H_u
\end{equation}
we derive an effective low energy Hamiltonian in the limit $|t_{ij}| \ll U$ up to 
third order. For taking account of the magnetic field the hoppings $t_{ij}$ can in 
general be complex. The effective Hamiltonian up to third order $H_{\text{eff}} = H_2 + H_3$
is given by
\begin{align}
  H_2 =  \frac{2}{U}\sum \limits_{\left<i, j\right>} &|t_{ij}|^2(P_{ij} -1) \\
  H_3 =  \frac{6}{U^2} \sum \limits_{i,j,k \in \triangle}&  i \text{Im}(t_{ij}t_{jk}t_{ki})(P_{ijk} -P_{ikj})  \\
             & - \text{Re}(t_{ij}t_{jk}t_{ki})(P_{ijk} + P_{ikj} - P_{ij} - P_{jk} - P_{ki} + 1)
\end{align}
where the two-site permutation operator is given by 
\begin{equation}
  \label{eq:twositesunperm}
  P_{ij} = \sum\limits_{\alpha,\beta} (c_{i\alpha}^\dagger c_{i\beta}) (c_{j\beta}^\dagger c_{j\alpha})
\end{equation}
 and the three-site permutation operator by 
\begin{equation}
  \label{eq:threesitesunperm}
  P_{ijk} = \sum\limits_{\alpha,\beta,\gamma} (c_{i\alpha}^\dagger c_{i\beta}) (c_{j\beta}^\dagger c_{j\gamma}) (c_{k\gamma}^\dagger c_{k\alpha})
\end{equation}
We notice that if the flux through the triangles is given by $\pi/2$ the real part 
of the third order effective Hamiltonian vanishes. More interestingly this 
part also vanishes in the case of SU($2$) since one can show that the identity
\begin{equation}
  \label{eq:sunthreetotwo}
  P_{ijk} + P_{ikj} = P_{ij} + P_{jk} + P_{ki} - 1
\end{equation}
holds for $N=2$ but not for $N>2$.

To derive the above results we perform a canonical transformation and project onto 
the sector with single site occupancy
\begin{equation}
  \label{eq:canonicaltrafo}
   H_{\text{eff}} = P_s e^{\eta} H e^{-\eta} P_s
\end{equation}
where the antiunitary operator
\begin{equation}
  \label{eq:schriefferwolf}
  \eta \equiv (P_dH_tP_s - P_s H_t P_d)/U
\end{equation}
fulfills $[\eta,H_U] = -H_t + P_dH_tP_d$, $P_s$ is the projector onto the subspace of single site occupancy and $P_d = 1 - P_s$.
Expanding eq.~\eqref{eq:canonicaltrafo} to third order yields
\begin{equation}
  \label{eq:canonicaltrafoexpansion}
  H_{\text{eff}} = H_U - \frac{1}{U}P_s H_t P_d H_t P_s  +  \frac{1}{U^2} P_s H_t P_d H_t P_d H_t P_s \dots 
\end{equation}
In the following we always assume that the color indices $\alpha, \beta$ and 
$\gamma$ are summed over. 
The second order effective Hamiltonian is now calculated as
\begin{align*}
  H_2 &\equiv - \frac{1}{U}P_s H_t P_d H_t P_s \\
         &= - \frac{1}{U}P_s\left(\sum \limits_{\left< i, j\right>} 
               t_{ij} c_{i,\alpha}^\dagger c_{j,\alpha} + t_{ij}^* c_{j,\alpha}^\dagger  c_{i,\alpha}\right)  P_d
           \left(\sum \limits_{\left< k, l\right> } t_{kl} c_{k,\beta}^\dagger c_{l,\beta} +
          t_{kl}^* c_{k,\beta}^\dagger  c_{l,\beta}\right) P_s \\
         &=  - \frac{1}{U}P_s\left( \sum \limits_{\left<i, j\right> } 
            t_{ij} t_{ij}^*c_{i,\alpha}^\dagger c_{j,\alpha} c_{j,\beta}^\dagger  c_{i,\beta} + 
            t_{ij}^* t_{ij} c_{j,\alpha}^\dagger  c_{i,\alpha} c_{i,\beta}^\dagger c_{j,\beta} \right)P_s\\
         &= - \frac{1}{U}P_s\left( \sum \limits_{\left<i, j\right>} 
             |t_{ij}|^2(1 - P_{ij}) +  |t_{ij}|^2(1 - P_{ji}) \right)P_s \\
         &= \frac{2}{U}P_s\left( \sum \limits_{\left<i, j\right>} 
             |t_{ij}|^2(P_{ij} -1) \right)P_s 
\end{align*}
The third order effective Hamiltonian is given by
\begin{equation}
  \label{eq:h3effdef}
  H_3 \equiv\frac{1}{U^2}P_s H_t P_d H_t P_d H_t P_s 
\end{equation}
The allowed processes up to third order take one fermion around a triangle
formed by nearest neighbour bonds. For every triangle we have twelve possibilities
how this can be achieved. For every site on the triangle a fermion can either hop clockwise
or counterclockwise around a triangle picking up a factor of $t_{ij}t_{jk}t_{ki}$ (resp. $t_{ij}^* t_{jk}^* t_{ki}^*$). Each of this six processes can be achieved in two ways: First hop 
a fermion from $i\rightarrow j$, then $j\rightarrow k$ and finally $k \rightarrow i$ or 
differently first $i\rightarrow j$, then $k \rightarrow i$ and finally $j\rightarrow k$.
This yields
\begin{align*}
   H_3 = -\frac{1}{U^2}t_{ij}t_{jk}t_{ki}\sum\limits_{i,j,k \in \triangle}&
  (c_{i,\alpha}^\dagger c_{j,\alpha})(c_{j,\beta}^\dagger c_{k,\beta})(c_{k,\gamma}^\dagger c_{i,\gamma}) + 
  (c_{i,\alpha}^\dagger c_{j,\alpha})(c_{k,\beta}^\dagger c_{i,\beta})(c_{j,\gamma}^\dagger c_{k,\gamma}) + \\
  &(c_{j,\alpha}^\dagger c_{k,\alpha})(c_{k,\beta}^\dagger c_{i,\beta})(c_{i,\gamma}^\dagger c_{j,\gamma}) + 
  (c_{j,\alpha}^\dagger c_{k,\alpha})(c_{i,\beta}^\dagger c_{j,\beta})(c_{k,\gamma}^\dagger c_{i,\gamma}) + \\
  &(c_{k,\alpha}^\dagger c_{i,\alpha})(c_{i,\beta}^\dagger c_{j,\beta})(c_{j,\gamma}^\dagger c_{k,\gamma}) + 
  (c_{k,\alpha}^\dagger c_{i,\alpha})(c_{j,\beta}^\dagger c_{k,\beta})(c_{i,\gamma}^\dagger c_{j,\gamma}) \\
  - \frac{1}{U^2} t_{ij}^*t_{jk}^*t_{ki}^*\sum\limits_{i,j,k \in \triangle} &
 (c_{j,\alpha}^\dagger c_{i,\alpha})(c_{k,\beta}^\dagger c_{j,\beta})(c_{i,\gamma}^\dagger c_{k,\gamma}) + 
  (c_{j,\alpha}^\dagger c_{i,\alpha})(c_{i,\beta}^\dagger c_{k,\beta})(c_{k,\gamma}^\dagger c_{j,\gamma}) + \\
  &(c_{k,\alpha}^\dagger c_{j,\alpha})(c_{i,\beta}^\dagger c_{k,\beta})(c_{j,\gamma}^\dagger c_{i,\gamma}) + 
  (c_{k,\alpha}^\dagger c_{j,\alpha})(c_{j,\beta}^\dagger c_{i,\beta})(c_{i,\gamma}^\dagger c_{k,\gamma}) + \\
  &(c_{i,\alpha}^\dagger c_{k,\alpha})(c_{j,\beta}^\dagger c_{i,\beta})(c_{k,\gamma}^\dagger c_{j,\gamma}) + 
  (c_{i,\alpha}^\dagger c_{k,\alpha})(c_{k,\beta}^\dagger c_{j,\beta})(c_{j,\gamma}^\dagger c_{i,\gamma}) 
\end{align*}
Using identities like 
\begin{equation}
  \label{eq:fermionstopermutation}
  (c_{i,\alpha}^\dagger c_{j,\alpha})(c_{j,\beta}^\dagger c_{k,\beta})(c_{k,\gamma}^\dagger c_{i,\gamma}) = 
  P_{ikl} - P_{ij} - P_{ik} + 1
\end{equation}
yields the result
\begin{align*}
   H_3 = &-\frac{1}{U^2}t_{ij}t_{jk}t_{ki}\sum\limits_{i,j,k \in \triangle}
            (6 P_{ikj} - 3 P_{ij}- 3 P_{jk}- 3 P_{ki} + 3)\\
            &- \frac{1}{U^2} t_{ij}^*t_{jk}^*t_{ki}^*\sum\limits_{i,j,k \in \triangle} 
            (6 P_{ijk} - 3 P_{ij}- 3 P_{jk}- 3 P_{ki} + 3) \\
  =&\frac{6}{U^2} \sum \limits_{i,j,k \in \triangle}  i \text{Im}(t_{ij}t_{jk}t_{ki})(P_{ijk} -P_{ikj})  \\
             & - \text{Re}(t_{ij}t_{jk}t_{ki})(P_{ijk} + P_{ikj} - P_{ij} - P_{jk} - P_{ki} + 1)
\end{align*}


==> chapters/introduction/symmetries.tex <==
%auto-ignore
\subsubsection{Internal symmetries}
\label{sec:internalsymmetries}

The discussion in the previous paragraph concerning the transition
from the classical Ising model to the quantum Heisenberg model in the
anisotropic Heisenberg model showed an order-to-disorder transition
between the classical and the quantum case. This transition can also
be interpreted differently. The symmetry group of the Ising model is
the discrete $\mathbb{Z}_2$ group for global spin flips. For the
isotropic Heisenberg case the symmetry group is enlarged to the
continuous SU($2$) spin rotation group. Thus the higher symmetric model
is fluctuating more than the lower symmetric model. The amount of
fluctuations can be increased by considering models with yet higher
symmetry group like a continuous SU($N$) group.
\todo{Explain this SU(N) shit}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../thesis"
%%% End:

